Flame: Simplifying Topology Extension in Federated Learning

Distributed machine learning approaches, including a broad class of federated learning (FL) techniques, present a number of benefits when deploying machine learning applications over widely distributed infrastructures. The benefits are highly dependent on the details of the underlying machine learning topology, which specifies the functionality executed by the participating nodes, their dependencies and interconnections. Current systems lack the flexibility and extensibility necessary to customize the topology of a machine learning deployment. We present Flame, a new system that provides flexibility of the topology configuration of distributed FL applications around the specifics of a particular deployment context, and is easily extensible to support new FL architectures. Flame achieves this via a new high-level abstraction Topology Abstraction Graphs (TAGs). TAGs decouple the ML application logic from the underlying deployment details, making it possible to specialize the application deployment with reduced development effort. Flame is released as an open source project, and its flexibility and extensibility support a variety of topologies and mechanisms, and can facilitate the development of new FL methodologies.

==> runtime.tex <==
\section{Runtime}

\todo{to be revisited. Work in progress...}
How components interact to achieve the reconfiguration of the system.


Given these components, the flame's workflow consists of several steps. The figure above is presented to aid the explanation of the steps.
Step 1: A user creates a machine learning job and submits it to the system (e.g., by using flamectl).
Step 2: The apiserver receives requests and forward it to the controller if requests appears to be valid.
Step 3: The controller takes the requests, takes actions, update state in database and returns responses back to the user.
Step 4: If the request is to start a job, the controller contacts a cluster orchestration manager(s) (e.g., kubernetes) and makes worker creation requests.
Step 5: The worker (e.g., container or pod) contains flamelet. Then, flamelet in the worker contacts notifier and waits for events.
Step 6: As soon as the worker creation is confirmed, the controllers send an event to each of the workers for the job via notifier.
Step 7: Once each worker receives an event on a task being assigned to it, it contacts the apiserver and fetches a manifest for the task.
Step 8: A manifest is comprised of two elements: ml code and configuration. The flamelet execute the task by creating a child process for the ml code.
Step 9: The flamelet monitors the execution of the task and updates the state once the task execution is over.
Step 10: In the meantime, the controller also monitors a job's status and take action when necessary (e.g., deallocating workers).

The above workflow can have some variations depending deployment mode. There are two types of deployment modes: orchestration and non-ochestration. In orchestration mode, all the workers are under the management of flame system through the help of cluster orchestrators. On the other hand, in non-orchestration mode, the workers of consuming data (e.g., training worker) are not under management of the flame system. The non-ochestration mode is useful in one of the following situations:
\begin{tightitemize}
	\item when the flame system doesn't have permission to utilize resources of geo-distributed clusters
	\item when the geo-distributed clusters are not under the management of one organization
	\item when participants of a FL job want to have a control over when to join or leave the job
\end{tightitemize}
In non-ochestration mode, the fleddge system is only responsible for managing (i.e., (de)allocation) non-data comsuming workers (e.g., model aggregating workers). The system supports a hybrid mode where some are managed workers and others are non-managed workers.

Note that the flame system is in active development and not all the functionalities are supported yet.


